Privacy Loss of Noise Perturbation via Concentration Analysis of A Product Measure

Noise perturbation is one of the most fundamental approaches for achieving $(\epsilon,\delta)$-differential privacy (DP) guarantees when releasing the result of a query or function $f(\cdot)\in\mathbb{R}^M$ evaluated on a sensitive dataset $\mathbf{x}$. In this approach, calibrated noise $\mathbf{n}\in\mathbb{R}^M$ is used to obscure the difference vector $f(\mathbf{x})-f(\mathbf{x}')$, where $\mathbf{x}'$ is known as a neighboring dataset. A DP guarantee is obtained by studying the tail probability bound of a privacy loss random variable (PLRV), defined as the Radon-Nikodym derivative between two distributions. When $\mathbf{n}$ follows a multivariate Gaussian distribution, the PLRV is characterized as a specific univariate Gaussian. In this paper, we propose a novel scheme to generate $\mathbf{n}$ by leveraging the fact that the perturbation noise is typically spherically symmetric (i.e., the distribution is rotationally invariant around the origin). The new noise generation scheme allows us to investigate the privacy loss from a geometric perspective and express the resulting PLRV using a product measure, $W\times U$; measure $W$ is related to a radius random variable controlling the magnitude of $\mathbf{n}$, while measure $U$ involves a directional random variable governing the angle between $\mathbf{n}$ and the difference $f(\mathbf{x})-f(\mathbf{x}')$. We derive a closed-form moment bound on the product measure to prove $(\epsilon,\delta)$-DP. Under the same $(\epsilon,\delta)$-DP guarantee, our mechanism yields a smaller expected noise magnitude than the classic Gaussian noise in high dimensions, thereby significantly improving the utility of the noisy result $f(\mathbf{x})+\mathbf{n}$. To validate this, we consider convex and non-convex empirical risk minimization (ERM) problems in high dimensional space and apply the proposed product noise to achieve privacy.

==> sections/discussion.tex <==
\section{Discussion}\label{sec:discussion}

\noindent\textbf{Comparison with Concentrated DP.}
The same PLRV definition is considered in Concentrated DP (CDP)~\cite{dwork2016concentrated,bun2016concentrated}, yet, CDP derives its tail bound using the moment generating function (MGF) of the PLRV. In contrast, in our work, we would like to clarify that our PLRV is proportional to $W \cdot U$, where $U$ is derived from a $\BP$ distribution that does not have an MGF.  Hence, it is not feasible to characterize our mechanism using CDP/zCDP, which requires the underlying PLRV to be sub-Gaussian and to admit an MGF. 
Given this limitation, we resort to deriving the tail bound of the PLRV using its $q$-th moments. An important conclusion in measure concentration theory is that the moment bound (which we adopted) for tail probability is always better than the ones derived using MGFs~\cite{philips1995moment}.  





